Estimating Product Cannibalisation in Wholesale using Multivariate Hawkes Processes with Inhibition

Product cannibalisation in the marketplace refers to the decrease in the sales of one product due to competition from another product. We examine this phenomenon in a wholesale data set provided by an international company. We use a multivariate Hawkes process where each product is represented by a dimension, with cross-inhibition effects that model product cannibalisation. To implement the Hawkes process with inhibition we resolve challenges regarding the integration of the intensity function and introduce a new, stronger conditions for stability as existing conditions are unnecessarily strict under inhibition. We conduct our analysis in a Bayesian framework, for which we design a dimension-independent prior on the cross-inhibition based on a reparametrisation.

==> BranchingOUTTAKES.tex <==


\section{Branching Structure with Inhibition} \label{appendix_branching}

This section outlines a sampling procedure that preserves the branching structure (see Section~\ref{subsec_branching}) of a Hawkes process, even if inhibition is present. 

 We define the direct parent of an event as follows. If $t_j$ is a direct offspring of $t_i$, then $t_i$ is the parents of $t_j$. For each event $t_i$ we define $B(t_i) =0$ if $t_i$ was an immigrant event. Otherwise $B(t_i)$ takes the index the direct parent of $t_i$. For example if $t_i$ has one offspring $t_j$ then $B(t_j) = i$. Moreover, let $C(t_i)$ contain all direct and indirect (`total') offsprings of $t_i$.

We assume that $\phi(x) = \max(0, x)$, as it ensures that $\lambda(t \, | \, \mathbf{K}^+) >\lambda(t \, | \, \mathbf{K}) $ for all $t$.

First, we review the classic thinning approach.

\begin{lemma} \label{lemma_thinning_sampler}
Let $X=(x_1 \dots x_P)$ be event times from a point process with intensity $\bar{\lambda}(\cdot)$. Suppose there is another point process with intensity function $\lambda(\cdot)$ such that $\bar{\lambda}(x) \geq \lambda(x)$ for all $x \geq 0$. To obtain samples from $\lambda(\cdot)$, take $X=(x_1 \dots x_P)$ as candidates. Let $Y$ be the empty set. Each $x_i$, $i = 1 \dots P$, is added to $Y$ with probability $\lambda(x_i) / \bar{\lambda}(x_i)$. The event times in $Y$ are samples from the process with intensity $\lambda(\cdot)$. 
\end{lemma}

This is the popular `thinning' sampler for point processes, as introduced by \citet{ogata_lewis_1981}. Algorithm~\ref{alg_without_branching} outlines this approach, where each event is thinned independently, regardless of the branching structure. In particular, in Line~\ref{algo_wot_original} we calculate $b_{original}$ using all generated events in $Y_{original}$, regardless how many of those are still in $Y$.

Now we look at a different sampling procedure as outlines in Algorithm~\ref{alg_branching}. It differs from the algorithm above in two aspects. Here, $b$ is calculated with only the retained events (Line~\ref{algo_wt_b}), and offsprings are removed with its parents (Line~\ref{algo_wt_remove}). Note that our sampling approach under inhibition is inherently different to the one introduced by \citet{apostolopoulou_mutually_2019} as they work with a different model set up that specifies inhibition through a multiplicative factor. 

\begin{theorem}
Algorithm~\ref{alg_branching} generates samples from the correct target intensity $\lambda(\cdot \, | \, \mathbf{K})$.
\end{theorem}

\begin{proof}
Before any event is removed, the algorithm mirrors the classic thinning approach.

Let us now assume that event $t_i$ is removed (Line~\ref{algo_wt_remove}), along with all of its offsprings, of which $k$ lie before event $t_j$, which remains. 
\begin{align*}
    Y_{original} & = (t_1 \dots t_{i-1}, t_i, t_{i+1} \dots t_{i+k}, t_j, \dots) \\
    Y & = (t_1 \dots t_{i-1}, t_j, \dots)
\end{align*}

Hence, at this point we could discard all events after $t_{i-1}$ and instead sample from any proposal (that is larger than the target) and thin again according to the classic thinning approach. We choose to sample this new proposal event from $\lambda(\cdot \, | \, \mathbf{K^+}, \mathcal{H} =Y )$ using the branching structure. However, we have already generated such an event, namely $t_j$. Since $t_j$ has not been removed, it was either an immigrant event or an offspring of an event in $Y$, therefore it can be viewed as sampled from the desired $\lambda(\cdot \, | \, \mathbf{K^+}, \mathcal{H} =Y )$. Hence, the ration in Line~\ref{algo_wt_ratio} follows the usual thinning procedure and Algorithm~\ref{alg_branching} describes a sampling procedure that samples from the target intensity function $\lambda(\cdot \, | \, \mathbf{K})$.
\end{proof}

Crucially, all parents of events in $Y$ are also in $Y$ by construction. Hence the branching structure is retained, even under inhibition. 


\begin{algorithm}[htb!]
\caption{Classic Thinning Sampling without branching structure}\label{alg_without_branching}
\begin{algorithmic}[1]
\State Sample $Y_{original} = (t_1 < \dots < t_N)$ from $\lambda(\cdot \, | \, \mathbf{K}^+)$ 
\State Set $Y = Y_{original}$
\For{$i$ in $1:N$}
    \State sample $u \sim \mathcal{U} [0, 1]$
    \State set $a = \lambda(t_i \, | \, \mathbf{K}, \mathcal{H} = Y )$
    \State set $b_{original} = \lambda(t_i \, | \, \mathbf{K^+}, \mathcal{H} =Y _{original} )$ \label{algo_wot_original}
    \If{$u > a/b_{original}$} 
        \State remove $t_i$ from $Y$
    \EndIf
\EndFor
\State Return $Y$ as a sample from the multivariate Hawkes Process
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[htb!]
\caption{Sampling with inhibition while retaining the branching structure}\label{alg_branching}
\begin{algorithmic}[1]
\State Sample $Y_{original} = (t_1 < \dots < t_N)$ from $\lambda(\cdot \, | \, \mathbf{K}^+)$ using branching
\State Keep the $B(t_i)$ for all $i = 1 \dots N$
\State Set $Y = Y_{original}$

\For{$i$ in $1:N$}
    \If {$t_i  \not\in Y $} next
    \Else{ sample $u \sim \mathcal{U} [0, 1]$}
        \State set $a = \lambda(t_i \, | \, \mathbf{K}, \mathcal{H} = Y )$
        \State set $b = \lambda(t_i \, | \, \mathbf{K^+}, \mathcal{H} =Y )$  \label{algo_wt_b}
        \If{$u > a/b$}  \label{algo_wt_ratio}
        \State remove $t_i$ and $C(t_i)$ from $Y$  \label{algo_wt_remove}
        \EndIf
    \EndIf
\EndFor
\State Return $Y$ as a sample from the multivariate Hawkes Process
\end{algorithmic}
\end{algorithm}

==> outtakes.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Sparsity} \label{subsec_sparse}


Many real life problems of multivariate Hawkes processes also contain sparsity in $\mathbf{K}$ \citep[e.g.][]{eichler_graphical_2017}. There are multiple successful cases of sparsity application available in the literature. \cite{xu_learning_2016} use group Lasso and the EM-Algorithm to uncover the entries of $\mathbf{K}$ that are truly zero. Two-step procedure are a common workaround to uncover those structural zeros. \cite{yu_hawkesian_2020} separate the learning of the structure and the estimation of the non-zero parameters. Similarly, \cite{miscouridou_modelling_2018} use elaborate hierarchical structures and prior specifications to uncover sparsity, heterogeneity, reciprocity, and community structure in their multivariate Bayesian estimation procedure. Both methods only provide an approximation to the parameters (or their posterior distributions).

Sparsity can aid the estimation of product cannibalisation in two ways. Firstly, two articles can be so dissimilar that they have no interaction and we would like to set these interactions to zero without any prepossessing. Secondly, even when articles are similar their interaction may be rather minor. In these cases the business insight is greater if such small interactions are set to zero and the focus lies on more sizeable interactions. Instead of having to find an arbitrary threshold the sparsity priors provide an elegant solution for this. 




\subsubsection{Sparsity Priors} \label{subsec_sparseprior}

Many real life problems of multivariate Hawkes processes contain sparsity (see Section~\ref{subsec_sparse}, which we wish to reflect in our model. As mentioned in Section~\ref{sec_priorchoice}, when $M$ is large, the positive entries of $\mathbf{K}$ have to be small in order to retain stability (according to \ref{c3new} in Section~\ref{sec_stability}). When employing shrinkage strategies in larger dimensions it can therefore be difficult to distinguish between small non-zero entries of $\mathbf{K}^{*}$ and truly zero ones. 

For our example we therefore choose to place regularised horseshoe priors independently on each $K^*_{ij}$, which shrink small values towards zero but induces only little shrinkage on larger values \citep{piironen_sparsity_2017}.

Let us write 
\begin{align}
     \tilde{\xi}_{ij}^{2}=\frac{c^{2} \xi_{ij}^{2}}{c^{2}+\tau^{2} \xi_{ij}^{2}}
\end{align}
which allows us to set up the regularised horseshoe prior as follows:
\begin{align}
    \xi_{ij} & \sim \text{Cauchy}(0, 1) \\
    \tau & \sim \text{Cauchy}(0, \tau_0^2) \\
    c^2 & \sim \text{Inv-Gamma}(\nu/2, \nu/2) \\ 
     K^*_{ij} & \sim \mathcal{N}(0,\tilde{\xi}_{ij} \, \tau \, s^2) & \text{ for } i,j = 1 \dots M & \text{ (stable only) }
\end{align}
where we choose $\tau_0^2 = 0.1$, $\nu = 4$, and $s^2 = 1$ as above. Again, there is no structural assumption for $\mathbf{K}^{*}$. 

